When Measurement Constraints Favor Quantum Computational Sensing for Stealthy Power-Grid Attack Detection

Power-grid defenses that rely on digital telemetry remain vulnerable to stealthy attacks that preserve plausible reported states while altering the underlying physical system. We study when Nitrogen-Vacancy (NV) sensing provides a useful independent physical channel, and when coherent processing before measurement adds value. Across IEEE 14-, 30-, and 118-bus simulations with Lindblad NV models, we evaluate standard FDIA, BDD-stealth, statistical-stealth, and concealed topology attacks. The results reveal an observability hierarchy: evidence shifts from digital telemetry, to reported-versus-physical consistency, to the physical NV state. Quantum Computational Sensing (QCS) follows this selectivity, becoming informative only when the physical state itself carries attack evidence. We then compare QCS, conventional 4-setting NV readout, and tomography under matched measurement budgets. At a matched total budget of only 40 physical trials per sensor on case14, QCS reaches AP $0.944$, versus 0.800 for conventional NV readout and 0.751 for tomography; the same low-budget ordering holds on case30 and case118. Multi-setting methods recover as additional measurements become affordable, showing that the QCS benefit is a measurement-efficiency advantage rather than a universal accuracy advantage. Finally, we ask where the benefit varies across the three case simulations. Although the quantum-to-classical Fisher-information ratio increases from 1.21x to 1.54x, Normal--Attack Helstrom separation collapses in the harder regimes, and interleaved control substantially increases that separation only on case14, thereby quantum sensitivity does not necessarily imply task-relevant distinguishability. Our results show that realized QCS utility depends on the full chain from physical perturbation to state separation, coherent processing, and measurement under the resource constraints of the task.

==> sections/checklist.tex <==
% \section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1--2 sentence) justification right after your answer (even for \answerNA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will also be asked to include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While \answerYes{} is generally preferable to \answerNo{}, it is perfectly acceptable to answer \answerNo{} provided a proper justification is given (e.g., error bars are not reported because it would be too computationally expensive'' or ``we were unable to find the license for the dataset we used''). In general, answering \answerNo{} or \answerNA{} is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

% %%% END INSTRUCTIONS %%%


% \begin{enumerate}

% \item {\bf Claims}
%     \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
%     \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: \justificationTODO{}
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
%         \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
%         \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
%         \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
%     \end{itemize}

% \item {\bf Limitations}
%     \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
%     \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: \justificationTODO{}
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
%         \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
%         \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
%         \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
%         \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
%         \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
%         \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
%         \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
%     \end{itemize}

% \item {\bf Theory assumptions and proofs}
%     \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
%     \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: \justificationTODO{}
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer \answerNA{} means that the paper does not include theoretical results. 
%         \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
%         \item All assumptions should be clearly stated or referenced in the statement of any theorems.
%         \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
%         \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
%         \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
%     \end{itemize}

%     \item {\bf Experimental result reproducibility}
%     \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
%     \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: \justificationTODO{}
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer \answerNA{} means that the paper does not include experiments.
%         \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
%         \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
%         \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
%         \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
%         \begin{enumerate}
%             \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
%             \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
%             \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
%             \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
%         \end{enumerate}
%     \end{itemize}


% \item {\bf Open access to data and code}
%     \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
%     \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: \justificationTODO{}
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer \answerNA{} means that paper does not include experiments requiring code.
%         \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
%         \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
%         \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
%         \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
%         \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
%         \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
%         \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
%     \end{itemize}


% \item {\bf Experimental setting/details}
%     \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
%     \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: \justificationTODO{}
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer \answerNA{} means that the paper does not include experiments.
%         \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
%         \item The full details can be provided either with the code, in appendix, or as supplemental material.
%     \end{itemize}

% \item {\bf Experiment statistical significance}
%     \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
%     \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: \justificationTODO{}
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer \answerNA{} means that the paper does not include experiments.
%         \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
%         \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
%         \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
%         \item The assumptions made should be given (e.g., Normally distributed errors).
%         \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
%         \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
%         \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
%         \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
%     \end{itemize}

% \item {\bf Experiments compute resources}
%     \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
%     \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: \justificationTODO{}
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer \answerNA{} means that the paper does not include experiments.
%         \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
%         \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
%         \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
%     \end{itemize}
    
% \item {\bf Code of ethics}
%     \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
%     \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: \justificationTODO{}
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
%         \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
%         \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
%     \end{itemize}


% \item {\bf Broader impacts}
%     \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
%     \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: \justificationTODO{}
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer \answerNA{} means that there is no societal impact of the work performed.
%         \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
%         \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
%         \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
%         \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
%         \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
%     \end{itemize}
    
% \item {\bf Safeguards}
%     \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
%     \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: \justificationTODO{}
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer \answerNA{} means that the paper poses no such risks.
%         \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
%         \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
%         \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
%     \end{itemize}

% \item {\bf Licenses for existing assets}
%     \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
%     \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: \justificationTODO{}
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer \answerNA{} means that the paper does not use existing assets.
%         \item The authors should cite the original paper that produced the code package or dataset.
%         \item The authors should state which version of the asset is used and, if possible, include a URL.
%         \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
%         \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
%         \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
%         \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
%         \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
%     \end{itemize}

% \item {\bf New assets}
%     \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
%     \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: \justificationTODO{}
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer \answerNA{} means that the paper does not release new assets.
%         \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
%         \item The paper should discuss whether and how consent was obtained from people whose asset is used.
%         \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
%     \end{itemize}

% \item {\bf Crowdsourcing and research with human subjects}
%     \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
%     \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: \justificationTODO{}
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
%         \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
%         \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
%     \end{itemize}

% \item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
%     \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
%     \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: \justificationTODO{}
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
%         \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
%         \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
%         \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
%     \end{itemize}

% \item {\bf Declaration of LLM usage}
%     \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
%     %this research? 
%     \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: \justificationTODO{}
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
%         \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
%     \end{itemize}

% \end{enumerate}

\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: The abstract and introduction state the paper's three
    scoped contributions: attack-dependent observability, a
    measurement-constrained regime favoring QCS, and the distinction between
    available quantum information and realized task performance. These claims
    are supported by RQ1--RQ3 and are explicitly presented as conditional
    rather than universal quantum advantage.

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: The Discussion explicitly addresses simulation
    rather than physical NV hardware, the trusted-sensor assumption,
    case14-only architectural ablations, and the non-deployability of
    cross-sensor coherent processing. Additional limitations and hardware
    sensitivity analyses are provided in the appendix.

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper is primarily empirical and does not
    introduce new theorems or formal theoretical guarantees. Fisher-information
    quantities and quantum-sensing relations are used as established
    diagnostics with appropriate references.

\item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: The System Model, Experimental Setup, and appendices
    specify the IEEE test systems, attack construction, NV dynamics,
    measurement protocols, QCS architecture, measurement budgets, evaluation
    metric, training configuration, and principal ablations needed to
    reproduce the main results.

\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{}
    \item[] Justification: The current submission does not provide a public
    anonymized code repository containing the complete experimental pipeline.
    The paper instead provides detailed methodological and experimental
    information intended to make the reported experiments reproducible.

\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: The Experimental Setup and supplementary experiments
    describe dataset construction and splits, sensing and measurement budgets,
    model configurations, optimization settings, interleaving depth, and
    evaluation procedures. Ablation-specific configurations are reported
    alongside their corresponding appendix results.

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: Experiments supporting the main cross-attack and
    cross-scale claims are reported as mean$\pm$standard deviation over three
    independent seeds. Diagnostic or computationally expensive single-run
    ablations are clearly identified as such rather than presented as
    multi-seed estimates.

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerNo{}
    \item[] Justification: All experiments were run on a CPU-based machine
    with 64 CPU cores and 64\,GB RAM, and representative training times are
    reported for the principal QCS configurations and scaling experiments.
    We do not provide per-run runtime or total compute consumption for every
    experiment.

\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: The work uses simulated power-system and quantum
    sensing experiments, involves no human subjects or personal data, and is
    presented as defensive cybersecurity research with explicit discussion of
    assumptions, deployment boundaries, and limitations.

\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}
    \item[] Justification: The Discussion addresses the potential benefit of
    independent physical sensing for protecting critical infrastructure while
    also emphasizing the limits of the proposed trust boundary, the risk of
    relying on an uncompromised sensing appliance, and the gap between
    simulation and deployable hardware.

\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not release a high-risk pretrained
    model, sensitive dataset, or other asset requiring controlled-access
    safeguards. The experiments use simulated grid and sensing data for a
    defensive detection task.

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper cites the external software, benchmark
    systems, and prior methods on which the experiments are based.

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}
    \item[] Justification: The current submission does not introduce or
    publicly release a new standalone dataset, pretrained model, or benchmark
    asset requiring separate asset documentation.

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}
    \item[] Justification: The work contains no crowdsourcing experiments or
    research involving human subjects.

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: The work does not involve human participants,
    personal data, or human-subject experimentation, so IRB review is not
    applicable.

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    \item[] Answer: \answerNA{}
    \item[] Justification: LLMs are not part of the paper's scientific methodology or experimental pipeline.

\end{enumerate}

==> sections/new_tables.tex <==
% ============================================================================
% Corrected/updated tables -- 2026-09-02
% Generated from the honest, shot-noise-corrected pipeline. See the
% accompanying HTML report (reports/qcs_interleaving_helstrom_analysis_2026-09-02.html)
% for the full investigation, including the bug that necessitated these
% corrections (a shot-noise asymmetry: several scripts trained/evaluated
% QCS's XGBoost combiner on noise-free oracle populations while
% Classical/Tomography's features correctly carried real finite-shot noise).
%
% Sources:
%   Table 1 (rq1-observability):  results/{case}_qcs_pivot/table1_consolidated_seed{42,43,44}.json
%                                  (SCADA-XGBoost, disc-B classifier, Physical NV state)
%                                  + results/multiseed_aggregate.json (Interleaved-QCS N=10,
%                                  already-established, never affected by the bug)
%                                  + verdict_triad_cta honest CTA numbers (already the
%                                  canonical source used elsewhere in the paper for the
%                                  Physical-NV-state CTA column specifically)
%   Table 2 (total-budget):       results/{case}_qcs_pivot/matched_total_budget_xgb.json
%                                  (native head column; FiniteShot-XGB; Tomography-XGB --
%                                  this script was NEVER affected by the bug)
%   Table 3 (qfi-performance):    results/{case}_qcs_pivot/quantum_interpretability_diagnostics.json
%                                  (F_Q/F_C, Helstrom -- unaffected by the bug) + Table 1's
%                                  corrected CTA numbers for Delta-AP
%   Table 4 (dataset-characteristics): dataset caches (B_actual, labels) + grid_config.py
% ============================================================================

% -----------------------------------------------------------------------
% TABLE 1: Attack-dependent observability, MERGED with the QCS
% readout/architecture breakdown (formerly Table 1b) across all 4 attacks.
% -----------------------------------------------------------------------
\section{new table}
\begin{table*}[t]
\centering
\caption{
Attack-dependent observability across IEEE case14, case30, and case118.
Values are Average Precision (AP). The first four rows per case
(SCADA-XGBoost, disc-$B$ classifier, Physical NV state, and Interleaved-QCS
Independent $N{=}10$ native/sigmoid) are mean$\pm$std over three independent
seeds -- \textbf{corrected from an earlier version}: the disc-$B$ classifier
and Physical NV state rows were recomputed with a consolidated,
honest-by-construction pipeline (\texttt{\_table1\_consolidated.py}) that
applies real finite-shot noise to \emph{both} the Ramsey and population
components of the classical readout (the previous version's
Physical-NV-state and disc-$B$ features used a cached array that stored
populations exact/noise-free -- a partially-oracle bug now fixed).
SCADA-XGBoost is unchanged (grid-level data only, never affected).
\textbf{Merged in from the former Table 1b}: the remaining five rows per
case give the full Interleaved-QCS readout/architecture grid --
Independent $N{=}1$/$N{=}10$ $\times$ native/sigmoid vs.\ XGBoost combiner,
plus Direct-POVM (a single trainable 2-outcome POVM
$M{=}V\mathrm{diag}(\sigma(\theta))V^\dagger$ whose outcome probability
$\mathrm{Tr}(M\rho)$ IS the prediction, no classical combiner at all) on the
entangling Tree-joint/Chain-joint architectures (all $K$ sensors fused into
one state before measurement -- not directly comparable in information
budget to the Independent per-sensor rows). These five rows are
\emph{single-seed point estimates} (\texttt{\_qcs\_readout\_all\_attacks.py},
seed 42, \textbf{the identical train/test split and scenario construction
used by \_table1\_consolidated.py for the first four rows}) run, per the
merge request, against \textbf{all four attacks}, not CTA alone -- treat
their precision accordingly relative to the 3-seed rows above them.
}
\label{tab:rq1-observability}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llcccc}
\toprule
Case & Method / channel &
Standard FDIA &
BDD-stealth &
Statistical-stealth &
CTA \\
\midrule

\multirow{9}{*}{case14}
& SCADA-XGBoost
& $\mathbf{1.000\pm0.000}$
& $0.501\pm0.003$
& $0.500\pm0.007$
& $0.505\pm0.003$ \\

& disc-$B$ classifier
& $0.709\pm0.055$
& $\mathbf{0.998\pm0.001}$
& $\mathbf{0.554\pm0.024}$
& $0.500\pm0.000$ \\

& Physical NV state (4-setting)
& $0.492\pm0.027$
& $0.478\pm0.009$
& $0.481\pm0.006$
& $0.995\pm0.002$ \\

& Interleaved-QCS Independent $N{=}10$, native/sigmoid
& $0.505\pm0.034$
& $0.502\pm0.016$
& $0.499\pm0.005$
& $0.982\pm0.005$ \\

& Interleaved-QCS Independent $N{=}10$, XGBoost
& $0.505$
& $0.459$
& $0.459$
& $\mathbf{0.998}$\textsuperscript{$\star$} \\

& Interleaved-QCS Independent $N{=}1$, native/sigmoid
& $0.578$
& $0.490$
& $0.515$
& $0.652$ \\

& Interleaved-QCS Independent $N{=}1$, XGBoost
& $0.484$
& $0.493$
& $0.496$
& $0.991$ \\

& Tree-joint $N{=}10$, Direct-POVM
& $0.481$
& $0.495$
& $0.491$
& $0.976$ \\

& Chain-joint $N{=}10$, Direct-POVM
& $0.496$
& $0.490$
& $0.490$
& $0.959$ \\

\midrule

\multirow{9}{*}{case30}
& SCADA-XGBoost
& $\mathbf{1.000\pm0.000}$
& $0.507\pm0.011$
& $0.506\pm0.014$
& $0.501\pm0.005$ \\

& disc-$B$ classifier
& $0.986\pm0.005$
& $\mathbf{1.000\pm0.000}$
& $0.509\pm0.002$\textsuperscript{$\dagger$}
& $0.500\pm0.000$ \\

& Physical NV state (4-setting)
& $0.497\pm0.009$
& $0.483\pm0.013$
& $0.500\pm0.007$
& $0.781\pm0.015$ \\

& Interleaved-QCS Independent $N{=}10$, native/sigmoid
& $0.497\pm0.011$
& $0.512\pm0.015$
& $0.506\pm0.009$
& $0.675\pm0.009$ \\

& Interleaved-QCS Independent $N{=}10$, XGBoost
& $0.541$
& $0.509$
& $0.496$
& $0.790$ \\

& Interleaved-QCS Independent $N{=}1$, native/sigmoid
& $0.522$
& $0.502$
& $0.541$
& $0.718$ \\

& Interleaved-QCS Independent $N{=}1$, XGBoost
& $0.499$
& $0.501$
& $0.512$
& $\mathbf{0.798}$\textsuperscript{$\star$} \\

& Tree-joint $N{=}10$, Direct-POVM
& $0.474$
& $0.498$
& $0.509$
& $0.695$ \\

& Chain-joint $N{=}10$, Direct-POVM
& $0.473$
& $0.499$
& $0.509$
& $0.693$ \\

\midrule

\multirow{9}{*}{case118}
& SCADA-XGBoost
& $\mathbf{1.000\pm0.000}$
& $0.450\pm0.009$
& $0.456\pm0.012$
& $0.500\pm0.004$ \\

& disc-$B$ classifier
& $0.996\pm0.001$
& $\mathbf{1.000\pm0.000}$
& $0.502\pm0.014$\textsuperscript{$\dagger$}
& $0.500\pm0.000$ \\

& Physical NV state (4-setting)
& $0.535\pm0.034$
& $0.490\pm0.006$
& $0.501\pm0.011$
& $0.763\pm0.013$ \\

& Interleaved-QCS Independent $N{=}10$, native/sigmoid
& $0.536\pm0.057$
& $0.495\pm0.010$
& $0.508\pm0.020$
& $0.680\pm0.007$ \\

& Interleaved-QCS Independent $N{=}10$, XGBoost
& $0.489$
& $0.500$
& $0.526$
& $0.774$ \\

& Interleaved-QCS Independent $N{=}1$, native/sigmoid
& $0.522$
& $0.496$
& $0.502$
& $0.703$ \\

& Interleaved-QCS Independent $N{=}1$, XGBoost
& $0.498$
& $0.492$
& $0.508$
& $\mathbf{0.775}$\textsuperscript{$\star$} \\

& Tree-joint $N{=}10$, Direct-POVM
& $0.551$
& $0.488$
& $0.500$
& $0.747$ \\

& Chain-joint $N{=}10$, Direct-POVM
& $0.520$
& $0.489$
& $0.491$
& $0.717$ \\

\bottomrule
\end{tabular}}

\vspace{2pt}
{\footnotesize \textsuperscript{$\dagger$}Statistical-stealth detection by the
disc-$B$ classifier collapses to chance level at scale once honestly
evaluated (case30: $0.780\!\to\!0.509$; case118: $0.902\!\to\!0.502$ from the
previous, partially-oracle version) -- a genuine negative finding, not
merely a smaller effect: the disc-$B$ classifier has essentially no
discriminative power against statistical-stealth attacks at case30/118
scale. It remains highly effective against BDD-stealth at all three scales.
\textsuperscript{$\star$}An XGBoost-combiner variant of Interleaved-QCS is
the single highest CTA value in its case block, edging out the 3-seed
Physical-NV-state row (case14: $0.998$ vs.\ $0.995$; case30: $0.798$ vs.\
$0.781$; case118: $0.775$ vs.\ $0.763$) -- flagged rather than bolded-as-final
because these are single-seed point estimates being compared against a
3-seed mean, and the margins at case30/118 ($+0.017$/$+0.012$) are well
within the $\pm0.009$--$0.02$ seed-to-seed spread seen elsewhere in this
table; case14's margin ($+0.003$) is negligible in absolute terms since both
readouts are already near-saturated ($>0.99$). \textbf{Reading the full
grid}: at case14, every readout choice converges to $\sim$0.98--0.99 on CTA
-- the trained state is close enough to Helstrom-orthogonal that readout
stops mattering (see the accompanying Helstrom analysis). At case30/118,
XGBoost recovers real gains over the native head at both $N{=}1$ and
$N{=}10$, and $N{=}1$ vs.\ $N{=}10$ become statistically indistinguishable
once XGBoost is the combiner -- interleaving earns its keep primarily by
making the native linear head usable, not by exposing information a
shallow rotation could not already expose to a strong classifier.
Direct-POVM (zero classical processing) is competitive with XGBoost at
case14 but trails it by $\sim$0.02--0.10 at case30/118. Against the other
three attacks, every Interleaved-QCS/Direct-POVM variant sits at chance
($\approx0.45$--$0.55$) at all three scales -- confirming this is a
CTA-specialized detector by architecture, not merely by the deployed
$N{=}10$/native configuration: swapping in XGBoost or Direct-POVM readout
does not surface any latent sensitivity to Standard FDIA, BDD-stealth, or
Statistical-stealth.}
\end{table*}


% -----------------------------------------------------------------------
% TABLE 2: Matched total physical measurement budget (EXTENDED to all 3 cases)
% -----------------------------------------------------------------------
\begin{table*}[t]
\centering
\caption{CTA detection under a matched total physical measurement budget,
all three grid scales, AP as a function of total measurement trials per
sensor $T$. \textbf{Two budget conventions are distinguished}: "matched
total budget" splits $T$ across each method's required settings (QCS-family:1,
4-setting:4, Tomography:7 -- so each setting gets fewer shots as the
setting count grows); "matched precision" instead gives every method's
\emph{each} setting $T$ shots (so classical/tomography use $4T$/$7T$ total
physical shots, not $T$) -- this isolates whether QCS's apparent
shot-efficiency comes from genuinely smarter use of a fixed budget, or
simply from needing fewer settings to split shots across. The "Settings"
and "Shots/setting" columns make this concrete for every row. The full
$N{\in}\{1,10\}\times\{$native,XGBoost$\}$ grid is shown for Interleaved-QCS
(Independent, per-sensor, no cross-sensor fusion), alongside
\textbf{Independent-direct} (per-sensor trainable POVM measurement, mean
across sensors, no fusion, no classical combiner) and Tree/Chain-joint
Direct-POVM (all $K$ sensors entangled into one state before the single
POVM measurement).
\textbf{Extended from case14-only to all three cases}; this pipeline was
never affected by the shot-noise bug (case118's row was regenerated once
more, after an unrelated CPU-usage fix, using a fresh noise realization --
same conclusions, slightly different point values than an earlier version
of this table).}
\label{tab:total-budget}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llclcccccc}
\toprule
Case & Method & Settings & Shots/setting & 40 & 200 & 400 & 1000 & 2000 & 20000 \\
\midrule

\multirow{11}{*}{case14}
& Interleaved-QCS $N{=}10$, native      & 1 & $T$   & $0.945$ & $0.981$ & $0.984$ & $0.985$ & $0.986$ & $0.986$ \\
& Interleaved-QCS $N{=}10$, XGBoost     & 1 & $T$   & $0.944$ & $0.986$ & $0.996$ & $0.998$ & $0.999$ & $0.999$ \\
& Interleaved-QCS $N{=}1$, native       & 1 & $T$   & $0.588$ & $0.653$ & $0.662$ & $0.675$ & $0.683$ & $0.693$ \\
& Interleaved-QCS $N{=}1$, XGBoost      & 1 & $T$   & $0.829$ & $0.938$ & $0.972$ & $0.987$ & $0.993$ & $0.996$ \\
& Independent-direct (POVM, no fusion)  & 1 & $T$   & $0.841$ & $0.851$ & $0.855$ & $0.856$ & $0.856$ & $0.857$ \\
& Tree-joint $N{=}10$, Direct-POVM      & 1 & $T$   & $0.972$ & $0.991$ & $0.992$ & $0.993$ & $0.993$ & $0.993$ \\
& Chain-joint $N{=}10$, Direct-POVM     & 1 & $T$   & $0.963$ & $0.982$ & $0.984$ & $0.986$ & $0.986$ & $0.986$ \\
& 4-setting NV (matched total budget)   & 4 & $T/4$ & $0.800$ & $0.956$ & $0.984$ & $0.991$ & $0.996$ & $0.996$ \\
& 4-setting NV (matched precision)      & 4 & $T$   & $0.945$ & $0.986$ & $0.987$ & $0.994$ & $0.993$ & $0.994$ \\
& Tomography (matched total budget)     & 7 & $T/7$ & $0.751$ & $0.935$ & $0.980$ & $0.993$ & $0.996$ & $0.999$ \\
& Tomography (matched precision)        & 7 & $T$   & $0.942$ & $0.994$ & $0.998$ & $0.999$ & $0.999$ & $0.9995$ \\
\midrule

\multirow{11}{*}{case30}
& Interleaved-QCS $N{=}10$, native      & 1 & $T$   & $0.684$ & $0.683$ & $0.672$ & $0.662$ & $0.640$ & $0.618$ \\
& Interleaved-QCS $N{=}10$, XGBoost     & 1 & $T$   & $0.608$ & $0.707$ & $0.759$ & $0.770$ & $0.818$ & $0.830$ \\
& Interleaved-QCS $N{=}1$, native       & 1 & $T$   & $0.666$ & $0.705$ & $0.706$ & $0.696$ & $0.697$ & $0.689$ \\
& Interleaved-QCS $N{=}1$, XGBoost      & 1 & $T$   & $0.586$ & $0.735$ & $0.770$ & $0.796$ & $0.828$ & $0.863$ \\
& Independent-direct (POVM, no fusion)  & 1 & $T$   & $0.537$ & $0.547$ & $0.577$ & $0.574$ & $0.583$ & $0.604$ \\
& Tree-joint $N{=}10$, Direct-POVM      & 1 & $T$   & $0.678$ & $0.718$ & $0.708$ & $0.709$ & $0.713$ & $0.699$ \\
& Chain-joint $N{=}10$, Direct-POVM     & 1 & $T$   & $0.644$ & $0.707$ & $0.720$ & $0.714$ & $0.708$ & $0.706$ \\
& 4-setting NV (matched total budget)   & 4 & $T/4$ & $0.514$ & $0.574$ & $0.662$ & $0.724$ & $0.743$ & $0.854$ \\
& 4-setting NV (matched precision)      & 4 & $T$   & $0.583$ & $0.727$ & $0.743$ & $0.784$ & $0.818$ & $0.864$ \\
& Tomography (matched total budget)     & 7 & $T/7$ & $0.526$ & $0.627$ & $0.666$ & $0.697$\textsuperscript{$\ddagger$} & $0.776$ & $0.855$ \\
& Tomography (matched precision)        & 7 & $T$   & $0.617$ & $0.732$ & $0.801$ & $0.826$ & $0.850$ & $0.885$ \\
\midrule

\multirow{11}{*}{case118}
& Interleaved-QCS $N{=}10$, native      & 1 & $T$   & $0.556$ & $0.627$ & $0.650$ & $0.675$ & $0.692$ & $0.724$ \\
& Interleaved-QCS $N{=}10$, XGBoost     & 1 & $T$   & $0.544$ & $0.664$ & $0.733$ & $0.774$ & $0.796$ & $0.816$ \\
& Interleaved-QCS $N{=}1$, native       & 1 & $T$   & $0.571$ & $0.671$ & $0.657$ & $0.706$ & $0.706$ & $0.732$ \\
& Interleaved-QCS $N{=}1$, XGBoost      & 1 & $T$   & $0.544$ & $0.682$ & $0.767$ & $0.767$ & $0.812$\rlap{$^\S$} & $0.819$ \\
& Independent-direct (POVM, no fusion)  & 1 & $T$   & $0.507$ & $0.510$ & $0.515$ & $0.514$ & $0.519$ & $0.531$ \\
& Tree-joint $N{=}10$, Direct-POVM      & 1 & $T$   & $0.537$ & $0.566$ & $0.602$ & $0.618$ & $0.642$ & $0.704$ \\
& Chain-joint $N{=}10$, Direct-POVM     & 1 & $T$   & $0.534$ & $0.605$ & $0.612$ & $0.648$ & $0.642$ & $0.708$ \\
& 4-setting NV (matched total budget)   & 4 & $T/4$ & $0.529$ & $0.521$ & $0.550$ & $0.653$ & $0.725$ & $0.806$ \\
& 4-setting NV (matched precision)      & 4 & $T$   & $0.567$ & $0.637$ & $0.716$ & $0.774$ & $0.786$ & $0.824$ \\
& Tomography (matched total budget)     & 7 & $T/7$ & $0.515$ & $0.532$ & $0.523$ & $0.646$ & $0.727$ & $0.806$ \\
& Tomography (matched precision)        & 7 & $T$   & $0.543$ & $0.667$ & $0.748$ & $0.783$ & $0.811$ & $0.813$ \\

\bottomrule
\end{tabular}}

\vspace{2pt}
{\footnotesize \textsuperscript{$\ddagger$}At $T{=}1000$, case30's
Tomography (matched-total-budget, 0.697) trails 4-setting NV readout (0.724)
slightly -- the ordering among classical baselines under the matched-total
convention is not perfectly monotonic in $T$ at this scale, unlike case14.
\textsuperscript{$\S$}case118's $N{=}1$+XGBoost column is non-monotonic
at $T{=}2000$ (single-run noise realization; not a systematic effect).
Reading the matched-precision columns: they consistently exceed their
matched-total-budget counterparts once settings $>$1 are involved (e.g.
case30 Tomography at $T{=}20000$: $0.885$ matched-precision vs $0.855$
matched-total-budget) -- confirming that some of QCS's apparent advantage
under a matched \emph{total} budget comes from needing to split shots
across fewer settings, not only from more informative per-shot readout;
under matched \emph{precision}, Tomography becomes the strongest method at
case30/118 by $T{=}20000$, consistent with \Cref{tab:rq1-observability}
and the main text's control-comparison discussion.}
\end{table*}


% -----------------------------------------------------------------------
% TABLE 3: QFI vs realized performance, WITH Helstrom columns added
% -----------------------------------------------------------------------
\begin{table}[t]
\centering
\caption{Quantum information versus realized QCS performance across scale.
$F_C$ denotes the Fisher information of the 4-setting NV readout and
$F_C^{\rm pop}$ that of a population-only measurement. $\Delta$AP is
Interleaved-QCS ($N{=}10$) minus 4-setting NV AP from
\Cref{tab:rq1-observability} (CTA column; unchanged from the original
table -- both numerator and denominator already used the honest CTA
values; computed from unrounded values, so it may differ by $\pm0.001$
from subtracting the table's rounded display figures directly). $D_Q^{\rm raw}$
is the Helstrom trace distance between class-averaged states \emph{before}
any control (the physical sensing state as produced by the Lindblad
evolution alone); $D_Q^{\rm post}$ is the same quantity \emph{after} the
trained $N{=}10$ interleaved control (both: mean across sensors, not
best-of-$K$); $P_{\rm Hel}=(1+D_Q^{\rm post})/2$ is the resulting
single-measurement discrimination bound on the post-training state.
\textbf{New: the three Helstrom columns} ($D_Q^{\rm raw}$, $D_Q^{\rm post}$,
$P_{\rm Hel}$), added to connect the Fisher-information argument
(estimation precision) to a genuine discrimination bound
(classification-relevant information), and to show explicitly how much
training moves the bound relative to where it started -- see
\S\ref{sec:helstrom-appendix} for the full per-sensor/pairwise/joint
breakdown.}
\label{tab:qfi-performance}
\begin{tabular}{lccccccc}
\toprule
Case & $F_Q/F_C$ & $F_Q/F_C^{\rm pop}$ & $\Delta$AP & $D_Q^{\rm raw}$ & $D_Q^{\rm post}$ & $P_{\rm Hel}$ & Training's effect \\
\midrule
case14  & $1.21\times$ & $4.7\times$ & $-0.013$ & $0.016$ & $0.229$ & $0.615$ & $+1332\%$ \\
case30  & $1.31\times$ & $6.2\times$ & $-0.106$ & $0.016$ & $0.016$ & $0.508$ & $+0.6\%$ \\
case118 & $1.54\times$ & $8.1\times$ & $-0.084$ & $0.003$ & $0.003$ & $0.501$ & $+3.4\%$ \\
\bottomrule
\end{tabular}

\vspace{4pt}
{\footnotesize Reading the added columns together with $\Delta$AP: at
case14, training the interleaved control moves the post-training Helstrom
bound substantially above chance ($P_{\rm Hel}{=}0.615$) even though
$\Delta$AP is near zero -- i.e., the realized classifier (Interleaved-QCS)
is already close to the classical-readout baseline, and the quantum state
itself has become meaningfully more discriminable than at the raw
(pre-control) level ($D_Q$ rises from $0.016$ to $0.229$, a $\sim\!14\times$
increase; see \S\ref{sec:helstrom-appendix}). At case30/118, $D_Q$ barely
moves from its raw baseline ($0.016\!\to\!0.016$; $0.003\!\to\!0.003$) --
training does not meaningfully reshape ensemble discriminability at these
scales, consistent with the larger negative $\Delta$AP (interleaved control
recovers less of the classical baseline's advantage) and with the smaller
$B$-field perturbations at these scales (\Cref{tab:dataset-characteristics}).
This is not a training failure: a single shared control unitary is
\emph{provably} unable to move $D_Q$ at all (it is the same fixed operator
for every sample, so it factors out of both class averages identically);
genuine interleaving ($N{\geq}2$) breaks this invariance only to the extent
that per-sample physics differs between classes, which is small when the
underlying field perturbation is small.}
\end{table}


% -----------------------------------------------------------------------
% TABLE 4: Dataset characteristics (NEW)
% -----------------------------------------------------------------------
\begin{table}[t]
\centering
\caption{Dataset characteristics across the three IEEE test-grid scales
used throughout this paper. Each case contains 5700 samples (3000 Normal,
1700 Fault [CTA source], 500 FDIA, 500 Cyber-Physical) with a 70/30
train/test split, identical across all three scales. $K$ is the number of
NV sensors. Effect size is the fault-induced shift in mean field magnitude
divided by the pooled standard deviation across samples (a
Cohen's-$d$-style measure) -- the field magnitude varies substantially
sample-to-sample regardless of fault status (loading conditions,
sensor-to-line geometry), so the raw mean shift alone is not an honest
measure of how detectable the fault is.}
\label{tab:dataset-characteristics}
\begin{tabular}{lccccccc}
\toprule
Case & Buses & Lines & $K$ & $|B|_{\rm normal}$ & $|B|_{\rm fault}$ & $\Delta|B|$ & Effect size \\
\midrule
case14  & 14  & 20  & 5  & 22020.91\,\textmu T & 26707.73\,\textmu T & 4686.82\,\textmu T & $0.230$ \\
case30  & 30  & 41  & 8  & 654.55\,\textmu T   & 682.30\,\textmu T   & 27.74\,\textmu T   & $0.067$ \\
case118 & 118 & 186 & 20 & 612.76\,\textmu T   & 613.17\,\textmu T   & 0.41\,\textmu T    & $0.001$ \\
\bottomrule
\end{tabular}

\vspace{4pt}
{\footnotesize Effect size collapses monotonically and steeply
($0.230\!\to\!0.067\!\to\!0.001$, roughly $3.4\times$ then $67\times$
smaller) -- not simply a function of grid scale or $K$ alone (case30 and
case118 differ $8\times$ in bus count and $2.5\times$ in $K$, yet their
effect sizes differ $67\times$, far more than either scale ratio). The
root cause is idiosyncratic to the standard benchmark topologies, not a
general law: pandapower's bundled \texttt{case14} network includes an
unusual 0.208\,kV low-voltage bus, which (since $P{=}VI$) forces very
large line currents there ($\approx$11.3\,kA mean) for a fixed real-power
flow, while case30/118 are purely transmission-level networks (1--345\,kV,
$\approx$0.16--0.19\,kA mean currents). This $\sim\!60$--$70\times$ current
disparity propagates linearly through the Biot--Savart field calculation
(identical, case-agnostic 0.10\,m sensor-to-line distance in all three
cases) into the observed field-magnitude gap. We report this plainly:
case14's favorable regime is a property of which standard IEEE benchmark
topology was used, not a general "smaller grids are easier to sense" law.}
\end{table}

% ============================================================================
% Appendix ablation: interleaving-depth (N) sweep, ALL THREE CASES
% Generated from the honest, shot-noise-corrected pipeline. See
% reports/qcs_interleaving_helstrom_analysis_2026-09-02.html (Section 3) for
% the case14-only discussion this table extends, and Section 11 for the
% shot-noise-asymmetry bug this script was fixed for.
%
% Source: results/{case}_qcs_pivot/interleaved_n{1,2,3,5,7,10}_shared_classifier.json
% (_interleaved_shared_classifier.py CASE N). Fixed 1000 shots/setting, CTA
% task, single seed per (case, N) run -- this answers "does interleaving
% depth itself matter, at a generous shot budget" rather than the
% shot-efficiency question (that is Table 2, tab:total-budget).
%
% 2026-09-03: extended from case14-only to all three cases (the N=2,3,5,7
% points were previously case14-only "by design" -- case30/118 only had the
% N=1/N=10 endpoints, already used elsewhere in the paper). This table now
% supersedes the case14-only version and the separate N=1-vs-N=10
% cross-case table (that comparison is now just the N=1/N=10 rows here).
%
% NOTE: these numbers come from a different single-seed script
% (_interleaved_shared_classifier.py, one run per N) than Table 1's
% Independent N=1/N=10 rows (_qcs_readout_all_attacks.py). Both measure the
% same underlying comparison and tell the same qualitative story, but are
% independent single-seed runs -- point values differ slightly (e.g. case30
% N=1+XGBoost: 0.809 here vs. 0.798 in Table 1, a ~0.01 discrepancy typical
% of single-seed noise between independently-trained runs). Do not merge
% into Table 1: the depth grid (N=2,3,5,7) has no counterpart there.
% ============================================================================

\begin{table}[t]
\centering
\caption{
Interleaving-depth ($N$) sweep, all three grid scales, CTA task, fixed
$1000$ shots/setting, native linear head vs.\ XGBoost combiner (both
trained on the multi-sensor concatenated population features). Single-seed
point estimates.
}
\label{tab:n-depth-sweep}
\begin{tabular}{llcc}
\toprule
Case & $N$ & Native head AP & + XGBoost AP \\
\midrule

\multirow{6}{*}{case14}
& 1  & $0.6640$          & $0.9918$ \\
& 2  & $0.8706$          & $0.9941$ \\
& 3  & $0.8949$          & $0.9933$ \\
& 5  & $0.9498$          & $0.9916$ \\
& 7  & $0.9696$          & $0.9942$ \\
& 10 & $\mathbf{0.9837}$ & $\mathbf{0.9982}$ \\
\midrule

\multirow{6}{*}{case30}
& 1  & $\mathbf{0.7112}$ & $0.8087$ \\
& 2  & $0.7087$          & $0.8198$ \\
& 3  & $0.6798$          & $\mathbf{0.8224}$ \\
& 5  & $0.6918$          & $0.8210$ \\
& 7  & $0.6920$          & $0.8195$ \\
& 10 & $0.6664$          & $0.7876$ \\
\midrule

\multirow{6}{*}{case118}
& 1  & $0.7100$          & $0.7821$ \\
& 2  & $0.6787$          & $\mathbf{0.7920}$ \\
& 3  & $0.7042$          & $0.7608$ \\
& 5  & $0.7017$          & $0.7771$ \\
& 7  & $\mathbf{0.7076}$ & $0.7621$ \\
& 10 & $0.6953$          & $0.7672$ \\

\bottomrule
\end{tabular}

\vspace{2pt}
{\footnotesize \textbf{case14}: the XGBoost ceiling is flat and already
saturated from $N{=}1$ onward ($0.992$--$0.998$); the \emph{native} head
rises smoothly and monotonically with $N$ ($0.664\to0.984$), still climbing
at $N{=}7\to N{=}10$ ($+0.014$) -- $N{=}10$ sits near, but not before, the
point of diminishing returns ($N{=}1\to N{=}2$ alone gains $+0.207$, more
than the entire $N{=}5\to N{=}10$ gain of $+0.034$). \textbf{case30/118}:
this monotonic story does \emph{not} replicate. Neither the native head nor
the XGBoost combiner rises with $N$ at either scale -- both fluctuate
within a narrow band ($\pm0.03$--$0.04$) with no consistent trend, and at
both cases $N{=}10$ is \emph{not} the best-performing depth for either
combiner (case30's best native head is $N{=}1$, $0.711$; case30's best
XGBoost is $N{=}3$, $0.822$; case118's best native head is $N{=}7$,
$0.708$; case118's best XGBoost is $N{=}2$, $0.792$ -- $N{=}10$ trails all
of these). This directly confirms, across the full depth grid rather than
just the two endpoints, that deeper interleaving does not unlock additional
separable information at case30/118 scale: whatever small differences exist
between depths there are consistent with single-seed noise around a flat
floor, not a genuine depth-dependent trend. The case14-specific "$N{=}10$
rescues a weak linear head" mechanism is therefore not a general property
of interleaving depth -- it depends on having a strong enough underlying
field perturbation (case14's difficulty-axis position, \Cref{tab:dataset-characteristics})
for depth to have anything to exploit in the first place.}
\end{table}

